25 Additional Problems -- Extension to the Book "125 Problems in Text Algorithms"

This very preliminary text is related to ``Algorithms on Texts'', also called ``Algorithmic Stringology''. It is an extension of the book ``125 Problems in Text Algorithms'' providing, in the same compact style, more problems with solutions. We refer also to the companions to ``Text algorithms'' available at http://monge.univ-mlv.fr/~mac/CLR/clr1-20.pdf and at the web page http://125-problems.univ-mlv.fr, where all 150 problems (including the ones presented here) are briefly announced. The selected problems satisfy three criteria: challenging, having short tricky solutions and solvable with only very basic background in stringology. For the basics in stringology we refer to http://monge.univ-mlv.fr/~mac/CLR/clr1-20.pdf.

==> pbs/extra-basics.tex <==

%\section*{Words}

In this chapter we introduce basic notations and ...

